Spontaneous gait synchronisation in the wild: exploring the effect of distance and level of interaction

Gait synchronization in pedestrians is influenced by biomechanical, environmental, and cognitive factors. Studying gait in ecological settings provides insights often missed in controlled experiments. This study tackles the challenges of assessing gait coordination in real-world interactions using a dataset of uninstructed pedestrian trajectories recorded in an underground pedestrian street network. The data are annotated for group relations, interaction levels, and physical contact. The main goals of our study is to devise a method to identify gait synchronisation from trajectory data and to provide an in-depth analysis of social factors affecting gait synchronisation in pedestrian groups. To that end, we first propose a method to extract gait residuals from pedestrian trajectories, which capture motion of the body caused by gait-induced oscillations. We thereafter apply a suite of analytical techniques spanning both frequency and nonlinear domains. Frequency-based methods, including the Gait Synchronisation Index and Cross Wavelet Coherence, quantify the alignment of oscillatory patterns in gait. Complementary nonlinear measures, such as Lyapunov exponents, determinism, and recurrence quantification metrics, offer deeper insights into the dynamical stability and predictability of coupled gaits. Results show that higher social interaction and closer distances enhance gait synchronization, reducing stride frequency variation and increasing stability. Additionally, triad formation and relative positioning are shown to influence synchronisation. Overall, our findings suggest that social interactions shape pedestrian gait coordination, with interaction level and distance being key factors.

==> tables/gait_stats_f.tex <==
\begin{table}

\centering
\caption{{\color{red}Mean value and standard deviation of velocity} $v$, stride frequency $f$, and stride length $l$ for different intensities of interaction. Kruskal-Wallis $p$-values for the difference between the intensities of interaction and Student's $t$-test $p$-values for the difference between all dyads and individuals are also shown.}
\label{tab:gait_stats}
\begin{tabular}{lcccccc}
\toprule
Intensity of interaction & \multicolumn{2}{c}{$v$ [m/s]} & \multicolumn{2}{c}{$f$ [Hz]} & \multicolumn{2}{c}{$l$ [m]} \\
\midrule
Interaction 0 & $1.30 \pm 0.17$ & \multirow{4}{*}{$\mathbf{< 10^{-4}}$} &$1.09 \pm 0.20$ & \multirow{4}{*}{$1.06 \times 10^{-1}$} &$1.51 \pm 0.69$ & \multirow{4}{*}{$\mathbf{< 10^{-4}}$} \\
Interaction 1 & $1.23 \pm 0.16$ & &$1.05 \pm 0.16$ & &$1.39 \pm 0.44$ & \\
Interaction 2 & $1.17 \pm 0.17$ & &$1.05 \pm 0.18$ & &$1.43 \pm 0.51$ & \\
Interaction 3 & $1.04 \pm 0.25$ & &$1.04 \pm 0.15$ & &$1.20 \pm 0.34$ & \\
\midrule
All & $1.18 \pm 0.20$ & &$1.05 \pm 0.18$ & &$1.41 \pm 0.52$ &\\
Individuals & $1.29 \pm 0.21$ & & $1.03 \pm 0.19$ & &$1.86 \pm 1.09$  & \\
\midrule
Student's $t$-test $p$-value & $\mathbf{< 10^{-4}}$ & &$1.80 \times 10^{-1}$ & &$\mathbf{< 10^{-4}}$ &\\
\bottomrule
\end{tabular}
\end{table}

==> tables/p_values_triads_formations.tex <==
\begin{table}
\centering
\caption{$p$-values for the Kruskal-Wallis tests for the independence of means of $\Delta f$, GSI and CWC for the different pairs in the triad, for all formations.}
\label{tab:p_values_triads_formations}
\begin{tabular}{lccc}
\toprule
Formation & $\Delta f$ & GSI & CWC \\
\midrule
$\vee$ & $4.16 \times 10^{-1}$ & $\mathbf{2.65 \times 10^{-2}}$ & $\mathbf{2.30 \times 10^{-3}}$ \\
$\wedge$ & $5.55 \times 10^{-1}$ & $8.75 \times 10^{-1}$ & $2.94 \times 10^{-1}$ \\
$\longleftrightarrow$ & $5.72 \times 10^{-1}$ & $1.19 \times 10^{-1}$ & $\mathbf{7.40 \times 10^{-3}}$ \\
\bottomrule
\end{tabular}
\end{table}


==> tables/tukey.tex <==
\begin{table}
\centering
\caption{Tukey's HSD test for pairwise comparisons of GSI between different intensities of interaction.}
\label{tab:tukey_gsi}
\begin{tabular}{lccccc}
\toprule
 & Baseline & Interaction 0 & Interaction 1 & Interaction 2 & Interaction 3 \\
\midrule
$B_r$ & - & $\mathbf{9.03 \times 10^{-4}}$ & $9.12 \times 10^{-1}$ & $9.66 \times 10^{-1}$ & $\mathbf{< 10^{-4}}$ \\
$B_c$ & - & - & $9.99 \times 10^{-1}$ & $9.56 \times 10^{-1}$ & $\mathbf{9.70 \times 10^{-4}}$ \\
Interaction 0 & - & - & - & $1.00$ & $2.59 \times 10^{-1}$ \\
Interaction 1 & - & - & - & - & $5.52 \times 10^{-2}$ \\
Interaction 2 & - & - & - & - & - \\
Interaction 3 & - & - & - & - & - \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}
\centering
\caption{Tukey's HSD test for pairwise comparisons of coherence between different intensities of interaction.}
\label{tab:tukey_coherence}
\begin{tabular}{lccccc}
\toprule
 & Baseline & Interaction 0 & Interaction 1 & Interaction 2 & Interaction 3 \\
\midrule
$B_r$ & - & $5.18 \times 10^{-2}$ & $8.72 \times 10^{-1}$ & $\mathbf{3.97 \times 10^{-3}}$ & $\mathbf{< 10^{-4}}$ \\
$B_c$ & - & - & $1.00$ & $1.14 \times 10^{-1}$ & $\mathbf{< 10^{-4}}$ \\
Interaction 0 & - & - & - & $6.09 \times 10^{-1}$ & $\mathbf{1.27 \times 10^{-3}}$ \\
Interaction 1 & - & - & - & - & $1.97 \times 10^{-1}$ \\
Interaction 2 & - & - & - & - & - \\
Interaction 3 & - & - & - & - & - \\
\bottomrule
\end{tabular}
\end{table}

